Unsupervised Keyphrase Extraction with Multipartite Graphs

We propose an unsupervised keyphrase extraction model that encodes topical information within a multipartite graph structure. Our model represents keyphrase candidates and topics in a single graph and exploits their mutually reinforcing relationship to improve candidate ranking. We further introduce a novel mechanism to incorporate keyphrase selection preferences into the model. Experiments conducted on three widely used datasets show significant improvements over state-of-the-art graph-based models.

==> _attic/ablation.tex <==
%\begin{table}[htb!]
%\centering
%\begin{tabular}{r|rrr}
%\toprule
%~ & \textbf{F@5} & \textbf{F@10} & \textbf{F@10} \\
%\midrule
%Full model               & 12.6 & 15.3 & 16.1 \\
%$-$\textsc{gwa}          & 11.0 & 13.7 & 14.3 \\
%$-$\textsc{OnePerTopic}  & 10.7 & 13.7 & 15.0 \\
%$-$\textsc{gwa}
%$-$\textsc{OnePerTopic}  & 9.1 & 12.2 & 13.3 \\
%\bottomrule
%\end{tabular}
%\caption{F-scores computed at the top 5, 10 and 15 extracted keyphrases.}
%\label{tab:ablation}
%\end{table}


\begin{table}[htb!]
\centering
\begin{tabular}{r|cc}
\toprule
~ & $+$\textsc{GWA} & $-$\textsc{GWA}  \\
\midrule
$+$\textsc{OnePerTopic}  & 16.1 & 14.3$^\dagger$\\
$-$\textsc{OnePerTopic}  & 15.0 & 13.3$^\dagger$ \\
\bottomrule
\end{tabular}
\caption{F-scores computed at the top 15 extracted keyphrases with or without graph weight adjustment (\textsc{GWA}), and with or without the one candidate per topic policy (\textsc{OnePerTopic}). $\dagger$ indicate significance at the 0.01 level using Student's t-test against our full model.}
\label{tab:ablation}
\end{table}

==> _attic/experiments.tex <==



We compare our proposed model against two baselines.
%
%
The first baseline is SingleRank~\cite{wan-xiao:2008:PAPERS}, a model in which keyphrase candidates are ranked by the sum of their words scores, computed using TextRank on a word-based graph representation.
%
In the latter, edges are weighted by the number of times two words co-occur in a fixed window of 10 words.
%
Because this model tends to suffer from over-generation errors~\cite{hasan-ng:2014:P14-1,boudin:2015:Keyphrase}, we also compute a modified version that normalizes candidate scores by their length as proposed in~\cite{boudin:2013:IJCNLP}.


\begin{enumerate}[label=$\bullet$, itemsep=.5em]

    \item \textbf{SemEval-2010 dataset}~\cite{kim-EtAl:2010:SemEval} which is composed of scientific articles collected from the ACM Digital Library.
    %\footnote{For the sake of reproducibility, we use the preprocessed version of the dataset made available by~\cite{boudin-mougard-cram:2016:WNUT}, \url{https://github.com/boudinfl/semeval-2010-pre/tree/master/test/lvl-2}}
    The dataset is divided into training (144 documents) and test (100 documents) sets.
    %
    We use the set of combined author- and reader-assigned keyphrases as reference keyphrases.
    
    \item \textbf{Hulth-2003 dataset}~\cite{Hulth:2003:IAK:1119355.1119383}, which is made of paper abstracts from about computer science and information technology.
    %
    The dataset is divided into training (1000 documents), development (500 documents) and test (100 documents) sets.
    %
    We use the set of professional indexer-assigned keyphrases as reference keyphrases.
    
    \item \textbf{Witten-1999 dataset}~\cite{Witten:1999:KPA:313238.313437}, that contains scientific articles from the Computer Science Technical Reports (CSTR) collection.
    %
    The dataset is divided into training (130 documents) and test (500 documents) sets.
    %
    We use the set of author-assigned keyphrases as reference keyphrases.
    
    %\item \textbf{Krapivin dataset}~\cite{krapivin2009large}, which is made of 2\,304 scientific articles collected from CiteSeerX.
    %
    %We preprocess each file with the Stanford CoreNLP suite~\cite{manning-EtAl:2014:P14-5}.
    %
    %For evaluation, we use the set of author-assigned keyphrases that were verified by reviewers.
    %Reference keyphrases were manually assigned by authors and verified by reviewers.

\end{enumerate}



The second baseline is TopicRank~\cite{bougouin-boudin-daille:2013:IJCNLP} which is the model that is closest to ours.
%
Additionally, we report a version without topical clustering, that is, which relies on a keyphrase candidate-based graph representation.
%
The rationale behind this modified version is to investigate the contribution of the topical information to the overall ranking.


TopicRank and the proposed model require one common parameter to be set: $\tau$, the similarity threshold for topic clustering.
%
Our model introduces one extra parameter, namely $\alpha$, that controls the strength of the graph weight adjustment.
%
These parameters are tuned on the training set of the SemEval-2010 dataset, and set to $\tau=0.9$ and $\alpha=1.0$ for all our experiments


%Our model requires two parameters to be set: $\tau$, the similarity threshold for topic clustering and $\alpha$, the parameter that controls the strength of the graph weight adjustment.
%
%These parameters are tuned on the training set, and set to $\tau=0.9$ and $\alpha=0.99$ for all our experiments.


%\subsection{Baselines}

%We compare our proposed model against two baselines.
%
%The first baseline is SingleRank~\cite{wan-xiao:2008:PAPERS}, a model in which keyphrase candidates are ranked by the sum of their words scores, computed using TextRank on a word-based graph representation of the document.
%
%The second baseline is TopicRank~\cite{bougouin-boudin-daille:2013:IJCNLP} which is the model that is closest to ours.
%
%In their model, documents are represented as a topic graphs in which topics are clusters of similar keyphrase candidates.
%
%Topics are then ranked using TextRank, and the first occurring candidate of the highest ranked topics are extracted.
%



%For reference, we also include a TF$\times$IDF $n$-gram based baseline as computed by the SemEval-2010 keyphrase extraction task organizers~\cite{kim-EtAl:2010:SemEval}.
%
%The latter is still a very strong baseline which was found to be on par with state-of-the-art unsupervised systems on the SemEval-2010 benchmark dataset~\cite{hasan-ng:2010:POSTERS,boudin-mougard-cram:2016:WNUT}.


%We conducted an ablation experiments
%In order to investigate the effect of the graph weight adjustment mechanism on candidate ranking, we compare two versions of our model: one with and one without graph weight adjustment ($-$\textsc{GWA}).
%
%We also analyse how topic coverage is affected by our one keyphrase per topic policy and conduct an ablation test in which multiple candidates per topic are allowed ($-$\textsc{OnePerTopic}).


\subsection{Results}

Results for the baselines and the proposed model are detailed in Table~\ref{tab:overall_results}.
%
Overall we observe that our model significantly outperforms both graph-based keyphrase extraction baselines.
%
Results are comparable across the datasets for F$_1$@5, and are somewhat lower on the Krapivin dataset for higher values of $N$.
%
This can be explained by the larger number of reference keyphrases per document in the SemEval-2010 dataset ($14.7$ compared to $5.3$ for the Krapivin dataset).


Comparing TopicRank with its version without topics, we see that topical information, although provided by a very simple clustering technique, is useful for ranking candidates.
%
Next, we observe that our model consistently improves over TopicRank, suggesting that it makes better use of the relations between topics and the candidates they instantiate.
%
With over $88\%$ of the top-10 extracted keyphrases assigned to different topics, our model successfully promotes topic coverage without the need of hard constraints. % as in previous models.
%
A manual inspection of a subset of `topic-redundant' keyphrases indicates that a good portion of these have in fact been wrongly assigned to the same topic. 


% indicates that most of the keyphrases that are in fact 
%[u'user queri', u'user']
%Dampening recommendations between intra-topic candidates also implicitely 


\section{Conclusion}

We introduced an unsupervised keyphrase extraction model that builds on a multipartite graph structure.
%
Our model allows for the seamless integration of any topical decomposition, and makes effective use of the mutually reinforcing relation between keyphrase candidates and topics.
%
We also proposed a graph weight adjustment mechanism to incorporate candidate selection preferences into the model. 
%
We demonstrated the effectiveness of our model on two publicly available datasets.


This paper reports work in progress and we would like to pursue two directions further.
%
First, the proposed multipartite graph representation opens up the possibility of applying tailored ranking algorithms, such as the one proposed in ().%~\cite{becker2013ranking}.
%
Second, our model should benefit from the use of more sophisticated topic decomposition methods, such as probabilistic topic models~(). %\cite{Hofmann:1999:PLS:312624.312649,Blei:2003:LDA:944919.944937}.

%It is important to note that the proposed model is language agnostic, making it particularly convenient for domains or languages where less data is available.
%
%This paper reports work in progress and we would like to pursue two directions further.
%In future work, we would like to pursue two directions.
%
%First, introducing a particular graph structure opens up the possibility of applying new ranking algorithms, for example the eigenvector-based algorithm proposed by~\newcite{becker2013ranking}.
%
%Second, as mentioned earlier, we rely on a very naive, lexically-based clustering approach to group keyphrase candidates into topics.
%
%Our model should really benefit from other topic decomposition methods, such as probabilistic topic models~\cite{Hofmann:1999:PLS:312624.312649,Blei:2003:LDA:944919.944937}.




%By introducing a new type of graph, namely a multipartite graph, our work opens up the possibility of applying type-specific ranking algorithms.
%
%In particular, the eigenvector-based ranking algorithm proposed by~\newcite{becker2013ranking} is relevant in the sense that it was shown to perform constantly better than other existing ranking on this type of graph.


%As mentioned previously, we use a very naive, lexically-based clustering approach to group keyphrase candidates into topics.
%
%Our model should really benefit from other topic decomposition methods, such as probabilistic topic models~\cite{Hofmann:1999:PLS:312624.312649,Blei:2003:LDA:944919.944937}.
%
%We leave exploration of such topic models to future work.





%Moreover, despite being limited to the content of the document, our model provide the same level of performance as TF$\times$IDF.
%
%This is particularly relevant for domains or languages where less data is available.


==> _attic/intro_ijcnlp2017.tex <==
Recent years have witnessed a resurgence of interest in automatic keyphrase extraction, and a number of diverse approaches were explored in the literature~\cite{kim-EtAl:2010:SemEval,hasan-ng:2014:P14-1}.
%
Among them, graph-based ranking approaches are appealing in that they offer strong performance and can be adapted in various ways, notably to represent diverse lexical units and their relations~\cite{mihalcea-tarau:2004:EMNLP,bougouin-boudin-daille:2013:IJCNLP,tixier-malliaros-vazirgiannis:2016:EMNLP2016}, to use information drawn from external resources~\cite{wan-xiao:2008:PAPERS,tsatsaronis-varlamis-norvrag:2010:PAPERS}, or to leverage training data~\cite{bougouin-boudin-daille:2016:COLING}.



In a nutshell, graph-based approaches to key-phrase extraction operate in two steps.
%
%First, the document is represented as a graph in which lexical units (words or phrases) act as nodes and the semantic relations among them as edges.
%
First, the document is represented as a graph where nodes are lexical units (words or phrases), and edges are semantic relations between them.
%
Second, a ranking algorithm is applied to estimate the importance of the lexical units, from which the top-ranked ones are selected as keyphrases.


%
Since the seminal work of \newcite{mihalcea-tarau:2004:EMNLP}, researchers have devoted a substantial amount of effort to develop better ways of modelling documents as graphs.
%
Most if not all previous work, however, focus on either measuring the semantic relatedness between nodes or devising node ranking functions.
%
So far, little attention has been paid to the use of different types of graphs for improving keyphrase extraction.
%
In this work, we explore this direction and propose a keyphrase extraction model that builds on a particular type of graph called multipartite graph.


Our contributions are twofold:
%
1)~we introduce a new multipartite graph-based representation model that allows for the seamless integration and proper use of any topical decomposition (\S\ref{subsec:multipartite}).
%
%2)~we provide a way to embed selection heuristics in the ranking process using graph weight adjustment (\S3).
2)~we provide a means for incorporating selection heuristics into the model by adjusting certain edge weights in the graph (\S\ref{subsec:graph-weight-adjustment}).


\section{Motivation}

A key challenge for keyphrase extraction systems is to produce a set of keyphrases that covers the main topics discussed in a document~\cite{liu-EtAl:2009:EMNLP1}.
%
This implies being able to group keyphrase candidates referring to the same topic, and to extract the candidates that best represents each topic.
%

Successful attempts at using topical information for graph-based keyphrase extraction typically involve biasing the ranking function towards topic distributions~\cite{liu-EtAl:2010:EMNLP1,zhao-EtAl:2011:ACL-HLT2011,zhang-huang-peng:2013:IJCNLP,xue-EtAl:2013:IJCNLP}.
%
%These models, however, aggregate multiple topic-biased rankings which makes their time complexity growing linearly with the number of topics.
%
These models, however, aggregate multiple topic-biased rankings which makes their time complexity prohibitive for long documents\footnote{Time complexity grows linearly with the number of topics, with optimal values ranging from $60$~\cite{zhang-huang-peng:2013:IJCNLP} to $1\,000$~\cite{liu-EtAl:2010:EMNLP1}.}.
%
%They also do not exploit the information provided by relations between topics.
They also do not exploit the semantic interactions between topics when ranking keyphrase candidates.

\input{img/vs-graph.tex}

Another strand of work proposes to model documents as graphs of topics and select keyphrases from the top-ranked ones~\cite{bougouin-boudin-daille:2013:IJCNLP}.
%
The idea is to use inter-topic relations, measured as the semantic relatedness between the candidates they instantiate, to improve the overall ranking (see Figure~\ref{fig:topicrank}).
%
The downside of this approach is that different candidates belonging to a single topic are viewed as equally important, so that post-ranking heuristics are applied to select the most representative candidates from each topic.


Here, we build upon this latter line of work and propose a model that enforces topical diversity while ranking keyphrase candidates in a single operation.
%
To do this, we use a multipartite graph structure to represent documents as tightly connected sets of topic related candidates.
%
Figure~\ref{fig:multipartite} shows an example of such a representation.



%\input{img/graph.tex}

%\begin{figure}[!htb]
%\centering
%\input{img/multipartite-graph.tex}
%\input{img/multipartite-graph.tex}
%\caption{Illustration of our multipartite graph representation for keyphrase extraction. Nodes are keyphrase candidates and edges represent co-occurrence relations.}
%\label{fig:graph}
%\end{figure}

Our model implicitly promotes the number of topics covered in the selected keyphrases by dampening intra-topic recommandation.
%
Encoding topical information within the graph allows the ranking function to make full use of the mutually reinforcing relation between topics and candidates.
%
Also, a benefit of ordering topic related candidates differentially is that the ones that best underpin each topic are directly given by the model.
%Although designed with a focus on simplicity, the multipartite graph-based representation of our model allows for efficient ranking and straightforward use of any topical decomposition.





%Similar to previous work, our model operate in two steps.
%
%First, a graph representation of the document is built where nodes are keyphrase candidates and edges are weighted using co-occurrence information.
%
%Second, a graph-based ranking algorithm is applied to assign a relevance score to each candidate.
%
%This section provides a detailed breakdown of these steps for our model.


For direct comparability with~\newcite{bougouin-boudin-daille:2013:IJCNLP}, which served as the starting point for the work reported here, we follow their setup for identifying keyphrase candidates and topics.
%
Keyphrase candidates are selected from the sequences of adjacent nouns and adjectives (\texttt{/(N|A)+/}).
%
They are then grouped into topics based on the stem forms of the words they share using hierarchical agglomerative clustering with average linkage.

\subsection{Multipartite graph representation}
\label{subsec:multipartite}


A complete directed multipartite graph is built, in which nodes are keyphrase candidates that are connected only if they belong to different topics.
%
Again, we follow~\cite{bougouin-boudin-daille:2013:IJCNLP} and weight edges according to the distance between two candidates in the document.
%
More formally, the weight $w_{ij}$ from node $i$ to node $j$ is computed as the sum of the inverse distances between the occurrences of candidates $c_i$ and $c_j$:
%
\begin{equation}
    w_{ij} = \sum_{p_i \in \mathcal{P}(c_i)}\ \sum_{p_j \in \mathcal{P}(c_j)} \frac{1}{|p_i - p_j|}
    \label{eq:edge-weighting}
\end{equation}
%
where $\mathcal{P}(c_i)$ is the set of the word offset positions of candidate $c_i$.


The resulting graph is a complete ${k}$-partite graph, whose nodes are partitioned into $k$ different independent sets, $k$ being the number of topics.
%
As exemplified in Figure~\ref{fig:vs-graph}, our graph representation differs from the one of~\cite{bougouin-boudin-daille:2013:IJCNLP} in two significant ways.
%
First, topics are encoded by partitioning candidates into sets of unconnected nodes instead of being subsumed in single nodes.
%
%this way, candidates are ranked 
% so that instead of grouping topic-related candidates 
% so that each candidate individually contribute 
% 
%
Second, edges are directed which, as we will see in the next section, allows to further control the incidence of individual candidates on the overall ranking.


Our model implicitly promotes the number of topics covered in the selected keyphrases by dampening intra-topic recommandation.
%
Encoding topical information within the graph allows the ranking function to make full use of the mutually reinforcing relation between topics and candidates.
%
Also, a benefit of ordering topic related candidates differentially is that the ones that best underpin each topic are directly given by the model.
%
%Although designed with a focus on simplicity, the multipartite graph-based representation of our model allows for efficient ranking and straightforward use of any topical decomposition.


\subsection{Graph weight adjustment mechanism}
\label{subsec:graph-weight-adjustment}

Selecting the most representative keyphrase candidates for each topic is a difficult task, and relying only on their importance in the document is not sufficient~\cite{hasan-ng:2014:P14-1}.
%
Among the features proposed to address this problem in the literature, the position of the candidate within the document is most reliable.
%
In order to capture this in our model, we adjust the incoming edge weights of the nodes corresponding to the first occurring candidate of each topic. 


More formally, candidates that occur at the beginning of the document are promoted according to the other candidates belonging to the same topic.
%
Figure~\ref{fig:gwa} gives an example of applying graph weight adjustment for promoting a given candidate.
%
Note that the choice of the candidates to promote, i.e.~the selection heuristic, can be adapted to fit other needs such that prioritising candidates from a controlled vocabulary.

\input{img/gwa.tex}

Incoming edge weights for the first occurring candidate of each topic are modified by the following equation:
%
\begin{equation}
w_{ij} = w_{ij} + \alpha \cdot \sum_{c_k \in \mathcal{T}(c_j) \setminus{\{c_j\}}} w_{kj}
\label{math:gwa}
\end{equation}
%
where $w_{ij}$ is the edge weight between nodes $c_i$ and $c_j$, $\mathcal{T}(c_j)$ is the set of candidates belonging to the same topic as $c_j$, and $\alpha$ is a hyper-parameter that controls the strength of the weight adjustment.

\subsection{Ranking and extraction}
\label{subsec:ranking}

After the graph is built, keyphrase candidates are ordered by a graph-based ranking algorithm, and the top $N$ are selected as keyphrases.
%
Here, we adopt the widely used TextRank algorithm~\cite{mihalcea-tarau:2004:EMNLP} in the form in which it leverages edge weights:
%
\begin{equation}
S(c_i) = (1 - \lambda) + \lambda \sum_{c_j \in \mathcal{I}(c_i)} \frac{w_{ij} \cdot S(c_j)}{\sum\limits_{c_k \in \mathcal{O}(c_j)}{w_{jk}}}
\label{math:textrank}
\end{equation}
%
where $\mathcal{I}(c_i)$ is the set of predecessors of $c_i$, $\mathcal{O}(c_j)$ is the set of successors of $c_j$, and $\lambda$ is a damping factor set to 0.85 as in~\cite{mihalcea-tarau:2004:EMNLP}.


%\subsection{Keyphrase extraction}
%
%Keyphrase candidates are ordered using the overall score of the topic they belong to (see Equation~\ref{math:topic_score}).
%
%This way, both candidate and topical importance are combined.

%\begin{equation}
%S^\prime(c_i) = \sum_{c_k \in \mathcal{T}(c_i)} S(c_k)
%\label{math:topic_score}
%\end{equation}
%\vspace{.3em}

%As stated by~\cite{liu-EtAl:2010:EMNLP1}, extracted keyphrases may fall into a single topic and fail to cover other substantial topics of the document.
%
%To avoid redundancy and maximise topic coverage, only one candidate -- the one with the highest score -- is extracted from each topic.


\section{Experiments}

\input{tables/results.tex}

\subsection{Datasets and evaluation measures}

%We carry out our experiments on the SemEval-2010 benchmark dataset~\cite{kim-EtAl:2010:SemEval}, which is composed of scientific articles collected from the ACM Digital Library.
%
%The dataset is divided into training (144 documents) and test (100 documents) sets.
%
%For the sake of reproducibility, we use the preprocessed version of the dataset made available by~\cite{boudin-mougard-cram:2016:WNUT}\footnote{\url{https://github.com/boudinfl/semeval-2010-pre/tree/master/test/lvl-2}}.


%As mentioned by (Hasan and Ng, 2010), it is essential to evaluate keyphrase extraction meth- ods on multiple datasets to fully understand their strengths and weaknesses.
%Experiments are carried out on two different datasets:
%
We carry out our experiments on two publicly available datasets:
%
\begin{enumerate}[label=$\bullet$, itemsep=.5em]
    \item \textbf{SemEval-2010 dataset\footnote{For the sake of reproducibility, we use the preprocessed version of the dataset made available by~\cite{boudin-mougard-cram:2016:WNUT}, \url{https://github.com/boudinfl/semeval-2010-pre/tree/master/test/lvl-2}}}~\cite{kim-EtAl:2010:SemEval}, which is composed of scientific articles collected from the ACM Digital Library.
    %
    The dataset is divided into training (144 documents) and test (100 documents) sets.
    %
    We use the set of combined author- and reader-assigned keyphrases as reference keyphrases.
    
    
    \item \textbf{Krapivin dataset}~\cite{krapivin2009large}, which is made of 2\,304 scientific articles collected from CiteSeerX.
    %
    We preprocess each file with the Stanford CoreNLP suite~\cite{manning-EtAl:2014:P14-5}.
    %
    For evaluation, we use the set of author-assigned keyphrases that were verified by reviewers.
    %Reference keyphrases were manually assigned by authors and verified by reviewers.
    
\end{enumerate}


We follow the common practice~\cite{kim-EtAl:2010:SemEval} and evaluate the performance of our method in terms of f-measure (F$_1$) at the top $N$ keyphrases, and apply stemming to reduce the number of mismatches.
%
%Stemming is applied to reduce the number of mismatches.
%We use the sets of manually assigned keyphrases as reference keyphrases,  
%We use the set of combined author- and reader-assigned keyphrases as reference keyphrases, and apply stemming to reduce the number of mismatches.


\subsection{Baselines and parameter settings}

We compare our proposed model against two baselines.
%
The first baseline is SingleRank~\cite{wan-xiao:2008:PAPERS}, a model in which keyphrase candidates are ranked by the sum of their words scores, computed using TextRank on a word-based graph representation.
%
In the latter, edges are weighted by the number of times two words co-occur in a fixed window of 10 words.
%
Because this model tends to suffer from over-generation errors~\cite{hasan-ng:2014:P14-1,boudin:2015:Keyphrase}, we also compute a modified version that normalizes candidate scores by their length as proposed in~\cite{boudin:2013:IJCNLP}.


The second baseline is TopicRank~\cite{bougouin-boudin-daille:2013:IJCNLP} which is the model that is closest to ours.
%
Additionally, we report a version without topical clustering, that is, which relies on a keyphrase candidate-based graph representation.
%
The rationale behind this modified version is to investigate the contribution of the topical information to the overall ranking.


TopicRank and the proposed model require one common parameter to be set: $\tau$, the similarity threshold for topic clustering.
%
Our model introduces one extra parameter, namely $\alpha$, that controls the strength of the graph weight adjustment.
%
These parameters are tuned on the training set of the SemEval-2010 dataset, and set to $\tau=0.9$ and $\alpha=1.0$ for all our experiments


%Our model requires two parameters to be set: $\tau$, the similarity threshold for topic clustering and $\alpha$, the parameter that controls the strength of the graph weight adjustment.
%
%These parameters are tuned on the training set, and set to $\tau=0.9$ and $\alpha=0.99$ for all our experiments.


%\subsection{Baselines}

%We compare our proposed model against two baselines.
%
%The first baseline is SingleRank~\cite{wan-xiao:2008:PAPERS}, a model in which keyphrase candidates are ranked by the sum of their words scores, computed using TextRank on a word-based graph representation of the document.
%
%The second baseline is TopicRank~\cite{bougouin-boudin-daille:2013:IJCNLP} which is the model that is closest to ours.
%
%In their model, documents are represented as a topic graphs in which topics are clusters of similar keyphrase candidates.
%
%Topics are then ranked using TextRank, and the first occurring candidate of the highest ranked topics are extracted.
%



%For reference, we also include a TF$\times$IDF $n$-gram based baseline as computed by the SemEval-2010 keyphrase extraction task organizers~\cite{kim-EtAl:2010:SemEval}.
%
%The latter is still a very strong baseline which was found to be on par with state-of-the-art unsupervised systems on the SemEval-2010 benchmark dataset~\cite{hasan-ng:2010:POSTERS,boudin-mougard-cram:2016:WNUT}.


%We conducted an ablation experiments
%In order to investigate the effect of the graph weight adjustment mechanism on candidate ranking, we compare two versions of our model: one with and one without graph weight adjustment ($-$\textsc{GWA}).
%
%We also analyse how topic coverage is affected by our one keyphrase per topic policy and conduct an ablation test in which multiple candidates per topic are allowed ($-$\textsc{OnePerTopic}).




\subsection{Results}

Results for the baselines and the proposed model are detailed in Table~\ref{tab:overall_results}.
%
Overall we observe that our model significantly outperforms both graph-based keyphrase extraction baselines.
%
Results are comparable across the datasets for F$_1$@5, and are somewhat lower on the Krapivin dataset for higher values of $N$.
%
This can be explained by the larger number of reference keyphrases per document in the SemEval-2010 dataset ($14.7$ compared to $5.3$ for the Krapivin dataset).


Comparing TopicRank with its version without topics, we see that topical information, although provided by a very simple clustering technique, is useful for ranking candidates.
%
Next, we observe that our model consistently improves over TopicRank, suggesting that it makes better use of the relations between topics and the candidates they instantiate.
%
With over $88\%$ of the top-10 extracted keyphrases assigned to different topics, our model successfully promotes topic coverage without the need of hard constraints. % as in previous models.
%
A manual inspection of a subset of `topic-redundant' keyphrases indicates that a good portion of these have in fact been wrongly assigned to the same topic. 


% indicates that most of the keyphrases that are in fact 
%[u'user queri', u'user']
%Dampening recommendations between intra-topic candidates also implicitely 


\section{Conclusion}

We introduced an unsupervised keyphrase extraction model that builds on a multipartite graph structure.
%
Our model allows for the seamless integration of any topical decomposition, and makes effective use of the mutually reinforcing relation between keyphrase candidates and topics.
%
We also proposed a graph weight adjustment mechanism to incorporate candidate selection preferences into the model. 
%
We demonstrated the effectiveness of our model on two publicly available datasets.


This paper reports work in progress and we would like to pursue two directions further.
%
First, the proposed multipartite graph representation opens up the possibility of applying tailored ranking algorithms, such as the one proposed in ().%~\cite{becker2013ranking}.
%
Second, our model should benefit from the use of more sophisticated topic decomposition methods, such as probabilistic topic models~(). %\cite{Hofmann:1999:PLS:312624.312649,Blei:2003:LDA:944919.944937}.

%It is important to note that the proposed model is language agnostic, making it particularly convenient for domains or languages where less data is available.
%
%This paper reports work in progress and we would like to pursue two directions further.
%In future work, we would like to pursue two directions.
%
%First, introducing a particular graph structure opens up the possibility of applying new ranking algorithms, for example the eigenvector-based algorithm proposed by~\newcite{becker2013ranking}.
%
%Second, as mentioned earlier, we rely on a very naive, lexically-based clustering approach to group keyphrase candidates into topics.
%
%Our model should really benefit from other topic decomposition methods, such as probabilistic topic models~\cite{Hofmann:1999:PLS:312624.312649,Blei:2003:LDA:944919.944937}.




%By introducing a new type of graph, namely a multipartite graph, our work opens up the possibility of applying type-specific ranking algorithms.
%
%In particular, the eigenvector-based ranking algorithm proposed by~\newcite{becker2013ranking} is relevant in the sense that it was shown to perform constantly better than other existing ranking on this type of graph.


%As mentioned previously, we use a very naive, lexically-based clustering approach to group keyphrase candidates into topics.
%
%Our model should really benefit from other topic decomposition methods, such as probabilistic topic models~\cite{Hofmann:1999:PLS:312624.312649,Blei:2003:LDA:944919.944937}.
%
%We leave exploration of such topic models to future work.





%Moreover, despite being limited to the content of the document, our model provide the same level of performance as TF$\times$IDF.
%
%This is particularly relevant for domains or languages where less data is available.


==> _attic/performances.tex <==
\begin{table}[htb!]
\centering
\begin{tabular}{r|rrr}
\toprule
\textbf{Model} & \textbf{F@5} & \textbf{F@10} & \textbf{F@15} \\
\midrule
SingleRank          &  2.5 &  3.4 &  4.8\\
TopicRank            & 10.0 & 12.6 & 13.7\\
%Multipartite ($-$\textsc{gwa}) & 11.0 & 13.7$^\dagger$ & 14.3\\
MultipartiteRank & \textbf{12.6}$^\dagger$ & \textbf{15.3}$^\dagger$ & \textbf{16.1}$^\dagger$\\
\midrule
TF$\times$IDF         & 11.9 & 15.9$^\dagger$ & 16.7$^\dagger$\\
\bottomrule
\end{tabular}
\caption{F-scores computed at the top 5, 10 and 15 extracted keyphrases. $\dagger$ indicate significance at the 0.01 level using Student's t-test against TopicRank.}
\label{tab:f-scores}
\end{table}


%\begin{table}[htb!]
%    \centering
%    \begin{tabular}{r|rrr}
%    \toprule
%    \textbf{Model} & \textbf{P} & \textbf{R} & \textbf{F} \\
%    \midrule
%    SingleRank       & 4.2  & 3.0 & 3.4\\
%    CandidateRank    & 15.0 & 10.6 & 12.3 \\
%    TopicRank        & 16.1 & 11.1 & 13.0 \\
%    MultipartiteRank-GWA & 14.8 & 10.4 & 12.1 \\
%    MultipartiteRank & 18.5 & 12.8 & 15.0 \\
%    \bottomrule
%    \end{tabular}
%    \caption{Caption}
%    \label{tab:results}
%\end{table}


==> _attic/results-bk.tex <==
%\begin{table*}[htb!]
%    \centering
%    \begin{tabular}{r|rrrrrr}
%    \toprule
%                 ~ & \multicolumn{3}{c}{\textbf{SemEval-2010}} & \multicolumn{3}{c}{\textbf{Krapivin}} \\
%    \textbf{Model} & \textbf{P} & \textbf{R} & \textbf{F} & \textbf{P} & \textbf{R} & \textbf{F} \\
%    \midrule
%    SingleRank~\cite{wan-xiao:2008:PAPERS} & 4.2  & 3.0 & 3.4   & 2.7 & 5.7 & 3.5 \\[.1cm]
    %CandidateRank    & 15.0 & 10.6 & 12.3 & - & - & - \\
%    TopicRank~\cite{bougouin-boudin-daille:2013:IJCNLP}        & 16.1 & 11.1 & 13.0 & 8.1 & 16.3 & 10.3 \\
%    $-$ topics        & 15.0 & 10.6 & 12.3 & - & - & - \\[.1cm]
%    MultipartiteRank & 18.5 & 12.8 & 15.0 & 9.3 & 18.7 & 11.8 \\
    %\midrule
    %TF$\times$IDF    & 19.9 & 14.0 & 16.3\\
%    \bottomrule
%    \end{tabular}
%    \caption{Caption}
%    \label{tab:overall_results}
%\end{table*}


\begin{table*}[htb!]
    \centering
    \begin{tabular}{r|rrr|rrr}
    \toprule
                 ~ & \multicolumn{3}{c}{\textbf{SemEval-2010}} & \multicolumn{3}{|c}{\textbf{Krapivin}} \\[.1cm]
    \textbf{Model} & \textbf{F$_1$@5} & \textbf{F$_1$@10} & \textbf{F$_1$@15} & \textbf{F$_1$@5} & \textbf{F$_1$@10} & \textbf{F$_1$@15} \\
    \midrule
    SingleRank             &  2.5 &  3.4 &  4.8 &  2.2 &  3.5 &  4.0 \\ %[.1cm] % ~\cite{wan-xiao:2008:PAPERS} 
    w/o over-generation errors                          &  8.9 & 10.2 & 11.5 &  8.5 &  9.1 &  8.5\\
    %\midrule
    \cmidrule(l{2pt}r{2pt}){1-1}
    \cmidrule(l{2pt}r{2pt}){2-4}
    \cmidrule(l{2pt}r{2pt}){5-7}
    TopicRank & 10.6 & 13.0 & 13.2 & 10.7 & 10.3 &  9.3 \\ %~\cite{bougouin-boudin-daille:2013:IJCNLP}
    %author's best parameters                            & 
    w/o topical clustering                              &  8.9 & 12.3 & 13.2 &  6.6 &  7.7 &  8.0 \\ %[.1cm]
    %\midrule
    \cmidrule(l{2pt}r{2pt}){1-1}
    \cmidrule(l{2pt}r{2pt}){2-4}
    \cmidrule(l{2pt}r{2pt}){5-7}
    Proposed model  & \textbf{11.4}$^\dagger$ & \textbf{14.9}$^\dagger$ & \textbf{15.5}$^\dagger$ & \textbf{12.0}$^\dagger$ & \textbf{11.9}$^\dagger$ & \textbf{10.8}$^\dagger$ \\
    %$-$ \textsc{gwa}  & 8.2 & 12.1 & 13.2 &   \\                                       
    %\midrule
    %TF$\times$IDF    & 19.9 & 14.0 & 16.3\\
    \bottomrule
    \end{tabular}
    \caption{F$_1$-scores computed at the top 5, 10 and 15 extracted keyphrases. $\dagger$ indicate significance at the 0.01 level using Student's t-test against TopicRank.}
    \label{tab:overall_results}
\end{table*}

==> _attic/results.tex <==

\begin{table*}[htb!]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{r|rrr|rrr|rrr}
    \toprule
        ~ &
        \multicolumn{3}{c}{\textbf{SemEval-2010}} &
        \multicolumn{3}{|c}{\textbf{Hulth-2003}} &
        \multicolumn{3}{|c}{\textbf{Witten-1999}}
    \\[.1cm]
        \textbf{Model} &
        \textbf{F$_1$@10} & \textbf{F$_1$@15} & \textbf{MAP} &
        \textbf{F$_1$@10} & \textbf{F$_1$@15} & \textbf{MAP} &
        \textbf{F$_1$@10} & \textbf{F$_1$@15} & \textbf{MAP} 
    \\
    \midrule
        CR~\cite{tixier-malliaros-vazirgiannis:2016:EMNLP2016}   
             &  7.3 &  7.2 & 20.7 
             &  4.5 &  4.6 & 11.2
             &  5.5 &  5.1 & 13.8 \\
             
        STPR~\cite{Sterckx:2015:TWI:2740908.2742730}
             &  9.6 &  9.9 & 21.5
             & 28.4 & \textbf{31.1} & 37.8
             &  6.8 &  6.3 & 16.4 \\
             
        PR~\cite{florescu-caragea:2017:Long} 
             & 11.7 & 11.5 & 26.2
             & 28.7 & 30.7 & 38.8
             &  9.6 &  8.7 & 20.6 \\
    
    \cmidrule(l{2pt}r{2pt}){1-1}
    \cmidrule(l{2pt}r{2pt}){2-4}
    \cmidrule(l{2pt}r{2pt}){5-7}
    \cmidrule(l{2pt}r{2pt}){8-10}
             
        TR~\cite{bougouin-boudin-daille:2013:IJCNLP}
             & 12.7 & 13.6 & 27.7
             & 28.4 & 28.9 & \textbf{47.0}
             &  9.5 &  8.7 & 19.7 \\
             
        w/o topical clustering
             & 12.2 & 13.2 & 23.6
             & 25.8 & 28.6 & 38.4
             &  9.0 &  8.9 & 16.9 \\
    
    \cmidrule(l{2pt}r{2pt}){1-1}
    \cmidrule(l{2pt}r{2pt}){2-4}
    \cmidrule(l{2pt}r{2pt}){5-7}
    \cmidrule(l{2pt}r{2pt}){8-10}
    
    Proposed model  & \textbf{14.7}$^\dagger$ & \textbf{16.4}$^\dagger$ & \textbf{27.9}
               & \textbf{29.6}$^\dagger$ & 30.8 & 44.1
               & \textbf{10.8}$^\dagger$ &  \textbf{9.9}$^\dagger$ & \textbf{20.8}$^\dagger$ \\

    \bottomrule
    \end{tabular}
    }
    \caption{F$_1$-scores computed at the top 10, 15 extracted keyphrases and Mean Average Precision (MAP) scores. $\dagger$ indicate significance at the 0.05 level using Student's t-test.}
    \label{tab:overall_results}
\end{table*}

